A Turbulence-Driven Magnetic Reconnection Model for the High-Energy Neutrino Emission from NGC 1068

We model the Seyfert II AGN NGC 1068 within a turbulence-induced magnetic reconnection framework to explain its high-energy emission. Observations reveal a neutrino flux excess higher than the observed GeV gamma-ray emission by orders of magnitude, with no detected TeV counterpart, suggesting efficient hadronic acceleration in the nuclear region with strong gamma-ray absorption. Assuming that proton acceleration occurs in a turbulent reconnection layer via a first-order Fermi process, we use a lepto-hadronic model based on a coronal-accretion disk configuration in which magnetic field lines anchored to the $2 \times 10^{7} M_{\odot}$ black hole horizon reconnect with field lines from the inner accretion disk corona. Our model matches the observed spectral energy distribution with a magnetic field $B_{c} \sim 10^{4}$ G and magnetic reconnection power $\dot{W_{B}} \sim 10^{43}$ erg s$^{-1}$, with $\sim 50\%$ efficiency in proton acceleration. Unlike previous studies, we find that both particle acceleration and emission take place in the inner region, where protons reach $\sim 10^{14}$ eV via first-order Fermi acceleration within the turbulent reconnection layer, rather than drift acceleration. These protons interact with disk photons, coronal X-rays, and coronal protons, producing neutrinos, predominantly via $pp$ interactions, at levels consistent with IceCube detections. The associated gamma-rays are attenuated by $\gamma\gamma$ annihilation, remaining below current upper limits. Turbulence-driven reconnection is thus a viable mechanism for neutrino production in the coronal region of NGC 1068 and similar sources.

==> table.tex <==
% \begin{table*}
%     \centering
%     \caption{Model Parameters of NGC 1068.}
%     \label{tablepartic}
%     \begin{tabular}{c cc cc}
%     \firsthline
%     \hline
%     Parameter & Name %& $N_{particles}$	
%     & Value & Reference \\
%     \hline
%     $m$  & Black Hole Mass ($M / M_{\odot }$) %& 50,000 
%     & $2 \times 10^{7}$ & \cite{zhang2021} \\ \\ 
    
%     RMHD-GACCEL    & 45 L/c	%&1,000 
%     & $3.5 \times 10^{-5}$	& $\sim 10^4$ hr.     \\ 
%     \lasthline
%     \end{tabular}
% \end{table*}

\begin{table*}
    \centering
    \caption{Model Parameters of NGC 1068.}
    \label{table_parameters}
    \begin{tabular}{c cc c cc}
    \firsthline
    \hline
    Parameter & Name & Value & Units & Reference \\
    \hline
    $m$ & Black Hole Mass & $2 \times 10^{7}$ & $M / M_{\odot }$ & \cite{zhang2021} \textcolor{red}{change all} \\
    $\dot{m}$ & Accretion Rate & 0.7 & $\dot{M} / \dot{M_{\rm Edd}}$ & \\
    $l$ & Coronal Magnetic Flux Tube Height & 10 & $L / R_{\rm Sch}$ & \\
    $l_{x}$ & Height of reconnection region & 10 & $L_{x} / R_{\rm Sch}$ & \\
    $r_{x}$ & Inner radius of disc & 10 & $R_{x} / R_{\rm Sch}$ & \\
    $B_{\rm 100\ pc}$ & Magnetic Field ($100$ pc from core) & $\sim 10^{-4}$ & G & \\
    $d$ & Distance & $\simeq 14410$ & kpc & \\
    $z$ & Redshift & $\sim 0.00379$ & & \\
    $v_{r}$ & Radial Velocity & $1137 \pm 3$ & km s$^{-1}$ & \\
    \hline
    $B_{c}$ & Coronal Magnetic Field & $1.05 \times 10^{4}$ & G & \\
    $n_{c}$ & Coronal particle number density & $3.44 \times 10^{10}$ & cm$^{-3}$ & \\
    $T_{c}$ & Coronal Temperature & $2.53 \times 10^{9}$ & K & \\
    $\Delta R_{X}$ & Width of the current sheet & $1.66 \times 10^{11}$ & cm & \\
    $\dot{W_{B}}$ & Reconnection Power & $5.99 \times 10^{42}$ & erg s$^{-1}$ & \\
    \lasthline
    \end{tabular}
\end{table*}


